An extension of data automata that captures XPath

We define a new kind of automata recognizing properties of data words or data trees and prove that the automata capture all queries definable in Regular XPath. We show that the automata-theoretic approach may be applied to answer decidability and expressibility questions for XPath.

==> classification.tex <==
{
\begin{table*}
%		\hspace{-0.3cm}
\begin{center}
		\begin{tabular}{l|l|l|l}
		\hline
		Model of counter  & % Restriction on 
		Class condition & Complexity of  & Languages of data  \\ 
		automata && emptiness & words captured \\
		\hline \hline
		Counter automata & No restriction & Undecidable & Extended Reg. XPath \\
		\hline
		Counter automata  & Local & Decidable, & Data automata,  \\
		w/o zero tests &&  EXPSPACE-hard & FO2($<,+1,\sim$) \\
		\hline
		Presburger automata & Commutatively  & NP-complete & FO2($+1,\sim$) \\
                & local && \\
		\hline
		Gainy counter  & Tail language & Decidable,  & Alternating one register  \\
		automata && non-primitive rec. & automata, \\
		&&& one register freeze LTL \\
		\hline
		\end{tabular}
	\caption{Classification of automata over data words.} \label{table:subclasses} 
\end{center}
\end{table*}
}

\section{Classification of automata on data words} \label{sec:classification} In this section, we show how all existing models of automata over data words can be presented as special cases of  class automata. In particular, we show how alternating one register automata~\cite{DBLP:journals/tocl/DemriL09} are captured by a restriction of class automata. 
%
We do the comparison for data words only. 

We also characterize expressibility of the relevant subclasses of class automata by (restrictions of)
counter automata.
%
%We work on binary trees, knowing that all the results transfer to unranked trees using the first child/next sibling encoding.


%(Although we do hope that  the decision procedure for alternating one register automata is easier 
%to follow when presented in terms of class automata.)


\sredniparagraph{Counter automata}  
Let $C$ be a finite set of 
 names for counters that  store natural numbers. A counter automaton is a nondeterministic finite state automaton, whose transitions, allowing also $\epsilon$-transitions, are labeled by counter operations. For each counter name $c$  we have the operations: increment ($c:=c+1$), decrement ($c:=c-1$) and zero test ($c=0?$). There are restrictions on executing  transitions labeled by decrement or zero test: for the decrement, the counter must have value at least $1$, for the zero test the counter must have value $0$. 
 A counter automaton accepts \marg{ok?} if in an accepting state all counters equal zero.
We write $\mathscr A_0$ for the class of counter automata. We identify the following subclasses of $\mathscr A_0$.
\begin{iteMize}{$\bullet$} 
	\item[$\mathscr A_1$:] Counter automata without zero tests.
	\item[$\mathscr A_2$:] Presburger automata. Counter values are in $\Int$. Only increments and decrements are allowed, and no zero tests. Decrements can always be executed. It is easy to encode this as a counter automaton, by representing an integer as the difference of two naturals.
	\item[$\mathscr A_3$:] Gainy counter automata. Like unrestricted counter automata, but each state must have a self-loop $\epsilon$-transition labeled by $c:=c+1$, for every $c \in C$.
\end{iteMize}
Unlike the unrestricted model, each of the three restricted models has decidable emptiness. For counter automata without zero tests, the underlying problem is reachability for vector addition systems, see~\cite{DBLP:conf/stoc/Mayr81}.
\marg{ok?}
For Presburger automata, the proof uses semilinear Parikh images. For gainy counter automata, the proof uses well-structured transition systems, see e.g.~\cite{DBLP:journals/tocl/DemriL09}.

\sredniparagraph{Restrictions on class condition} 
Recall the ingredients of a class automaton: a transducer $f$ from the input alphabet $\Sigma$ to the work alphabet $\Gamma$, and a class condition, which is a regular language $L$ over the alphabet $\Gamma \times \set{0,1}$. We write $\mathscr C_0$ for all class automata. 
  We identify three  restrictions on the class condition $L$, 
  which limit the way it inspects a word $w \otimes X$, with $w \in \Gamma^*$ and  $X$ a set of positions in $w$.
  They yield three subclasses of class automata:
\begin{iteMize}{$\bullet$}
	\item[$\mathscr C_1$:] The class condition $L$ is \emph{local}, i.e.,
	 membership $w \otimes X \in L$ depends only on the labels of positions $x \in X$. 
	 It does not depend on labels of positions outside $X$. 
	\item[$\mathscr C_2$:] The class condition is \emph{commutatively local}, i.e.,
	 membership $w \otimes X \in L$ depends only on the multiset 
	\begin{align*}
		 \set{w|Y : Y \mbox{ is a maximal interval contained in $X$}} \subseteq \Gamma^*.
	\end{align*}
	In the above, we write $w|Y$ for the substring of  $w$ corresponding to positions from $Y$. An interval means a connected set of positions.
	\item[$\mathscr C_3$:] The class condition is a \emph{tail language}, i.e., 
	there is a regular language $K$ such that 
	% for any word $w \otimes X$,    
	$w \otimes X \in L$ if and only if $K$ contains every suffix of $w \otimes X$ that begins in a position from $X$. 
\end{iteMize}
In the sequel we prove that $\mathscr C_1$ is equivalent to the model of data automata from~\cite{BojanczykLICS06}. 
We also show that $\mathscr C_3$ captures alternating one register automata 
% from~\cite{DBLP:journals/tocl/DemriL09} 
(the proof also works for trees).
In consequence $\mathscr C_3$ captures weak two-pebble automata~\cite{DBLP:journals/tocl/NevenSV04},
as they are simulated by alternating one register automata~\cite{DBLP:conf/mfcs/Tan09}.
The same applies to the top view weak pebble automata introduced in~\cite{DBLP:conf/mfcs/Tan09}.

\removed{\begin{enumerate}
	\item[1a.] $L$ is \emph{class local} if membership $w \otimes X \in L$ depends only on the labels of positions $x \in X$. It does not depend on labels of positions outside $X$. 
	\item[1b.] $L$ is \emph{strongly class local} if membership $w \otimes X \in L$ depends only on the sequence $w[X_1], \ldots, w[X_n]$. 
	\item[1c.] $L$ is \emph{very strongly class local} if membership $w \otimes X \in L$ depends only on $w[X] = w[X_1] \ldots w[X_n]$. 
	\item $L$ is \emph{commutatively class local} if membership $w \otimes X \in L$ depends only on the set $\set{w[X_1], \ldots, w[X_n]}$. 
	\item $L$ is a \emph{tail language} if there is a regular language $K$ such that 
	
	% for any word $w \otimes X$,    
	$w \otimes X \in L$ if and only if $K$ contains every suffix of $w \otimes X$ that begins in a position from $X$. 
\end{enumerate}}

\sredniparagraph{Classification} 
We will show that the restrictions on counter automata match the restrictions on class conditions. To compare languages of words without data and languages of data words, we use the following definition. Let $L$ be a set of data words over an alphabet $\Sigma$, and $\pi : \Sigma \to \Gamma \cup \set\epsilon$  a relabeling of $\Sigma$ that may erase some letters. We define $\pi(L) \subseteq \Gamma^*$ to be  the words without data obtained from $L$ by ignoring the data and applying $\pi$ to the underlying word. Any such language $\pi(L)$ is called a projection of $L$.




\begin{theorem}[Classification theorem]\label{thm:classification} For $i \in \set{0,1,2,3}$ the following language classes are equal:
	\begin{iteMize}{$\bullet$}
		\item Languages of words without data recognized by counter automata from $\mathscr A_i$.
		\item Projections of languages of data words recognized by class automata from  $\mathscr C_i$.
	\end{iteMize}
\end{theorem}

The translations in both directions are effective in the following sense. 
For any automaton $\Aa \in \mathscr A_i$, one can compute an automaton $\Cc \in \mathscr C_i $ 
and a projection $\pi$ such that the language of $\Aa$ is the projection under $\pi$ of the language of $\Cc$. 
Conversely, for any $\Cc \in \mathscr C_i$ and  $\pi$, one can compute an automaton $\Aa \in \mathscr A_i$ 
recognizing the projection under $\pi$ of the language of $\Cc$. 
Consequently, the  emptiness problems for $\mathscr A_i$ and $\mathscr C_i$ can be reduced to each other.
In most of the cases the reductions are polynomial.

The theorem is illustrated in Table~\ref{table:subclasses}. In the third column, the table  
includes the complexities of deciding emptiness for the counter automata.  
% , and therefore also the automata on data words. 
In the last column, the table lists some properties of data words  captured by the automata.

The table does not include nondeterministic automata with multiple registers of~\cite{KaminskiF94}. Their projections are regular word languages.  By~\cite{BjorklundS07} we know that nondeterministic register automata are captured by data automata, and therefore they correspond to some restriction on the class condition in a  class automaton.  But the construction in~\cite{BjorklundS07} is quite sophisticated, and we do not know what this restriction is.

We are curious how our undecidable model over data words and trees relates to other undecidable models, such as 
strong one-way pebble automata,
alternating automata with multiple registers, or two-way automata with registers, or combinations thereof.


The remaining part of this section is devoted to the proof of Theorem~\ref{thm:classification}. Most of the proof is standard, and uses known results from~\cite{DBLP:journals/tocl/DemriL09}, \cite{BojanczykJACM09} and~\cite{BojanczykLICS06}. There are two original contributions: a) we show that data automata are the same as class automata with a local class condition; b) we show that alternating one register automata are captured by class automata with tail class conditions.


\subsection{$\mathscr A_0$ versus $\mathscr C_0$}
We begin by considering the general case, which involves the powerful  but undecidable automata: counter automata and class automata.

\begin{proposition}
\label{prop:A0vsC0}
The following language classes are equal.
	\begin{enumerate}
		\item Languages of words without data recognized by counter automata.
		\item Projections of languages of data words recognized by class automata.
	\end{enumerate}
\end{proposition}
\begin{proof}(sketch)
	We begin with the inclusion of the first class in the second class.
	Consider a counter automaton with the set of transitions $\Delta$.	
	Let $L$ be a language over alphabet $\Delta$ that contains all data words $(w,\sim)$ 
such that the following condition holds.
	\begin{quote} Let $x$ be a position  with label $c:=c+1$. Then there is exactly one other position $y$ in the same class, this position is after $x$, and has label $c:=c-1$. Furthermore, no position between $x$ and $y$ is labeled by the test $c=0$.
	\end{quote}
	The language $L$ is recognized by a class automaton. It is not difficult to see that after erasing the data values from $L$, we get exactly the accepting runs of the counter automaton. Consequently, the language accepted by the counter automaton is obtained from $L$ by erasing data values and projecting each transition onto the letter it reads.
	
	The opposite inclusion, of the second class in the first class, is proved the same way as when translating a data automaton into a counter automaton without zero tests in~\cite{BojanczykLICS06}. The zero tests are used to capture the additional power of class automata.
\end{proof}


% \begin{proof}

\subsection{$\mathscr A_1$ versus $\mathscr C_1$}
We  move to the first of the three decidable restrictions: counter automata without zero tests, and class automata with local class conditions. Case $i=1$ of Theorem~\ref{thm:classification} follows now from the two results below, which use data automata~\cite{BojanczykLICS06}. Before we define data automata, we state the two results.

\begin{proposition}\label{prop:data-petri}The following language classes are equal.
	\begin{enumerate}
		\item Languages of words without data recognized by counter automata without zero tests.
		\item Projections of languages of data words recognized by data automata.
	\end{enumerate}
\end{proposition}

\begin{proposition}\label{prop:local-data}
	Data automata and class automata with local class conditions recognize the same languages of data words.	
\end{proposition}

Proposition~\ref{prop:data-petri} was shown in~\cite{BojanczykLICS06}. We now define a data automaton  and prove Proposition~\ref{prop:local-data}.

A \emph{data automaton} is given by a transducer and a class condition. The transducer is the same as in a class automaton, it is a letter-to-letter transducer $f: \Sigma^* \to \Gamma^*$ from the input alphabet $\Sigma$ to the work alphabet $\Gamma$. The difference is in the class condition: in a data automaton the class condition is a language $L \subseteq \Gamma^*$ over the work alphabet $\Gamma$, and not over $\Gamma \times \set{0,1}$. A data word $(w,\sim)$ is accepted if there is an output $v \in f(w)$ of the transducer such that for every class $X$, the string $v |X$ belongs to $L$.

Clearly a data automaton is a special case of a class automaton with a local class condition. The interest of Proposition~\ref{prop:local-data} is that each automaton with a local class condition is equivalent to a data automaton. We show this below.


Consider a class automaton, with transducer $f$ and a local class condition $L$.
Let $X$ be a set of positions. The $X$-successor of $x$ is the first position after $x$ in $X$. This position may be undefined, written as $\bot$.
For $n \in \Nat$,  the $n$-profile of a position  $x$ with respect to a set $X$  is a symbol in
	\begin{align*}
		\Pi_n = \set{\bot,+1,\ldots,+n, \mod 1, \ldots, \mod n}
	\end{align*} 
defined as follows.
If $x$ has no $X$-successor, the symbol is $\bot$.
Otherwise, let $d$ be the distance between $x$ and its $X$-successor;
if $d$ is at most $n$, then the symbol is $+d$; otherwise the symbol is$\mod d'$, where 
$d' \in \{1, \ldots, n\}$ and $d' \equiv d \mod n$.	

The  $n$-profile of data word $(w,\sim)$ is defined to be the function that maps each position of $w$  to its $n$-profile with respect to its own class. The $n$-profile can be treated as a word $v \in \Pi_n^*$ of the same length as $w$.
	
Proposition~\ref{prop:local-data} follows from the following two lemmas, and closure of data automata under relabelings and intersections.  The second lemma follows  from~\cite{BjorklundS07}.
\begin{lemma}
	Let $L \subseteq (\Gamma \times \set{0,1})^*$ be a local language. There is some $n \in \Nat$ and a regular language $K \subseteq (\Gamma \times \Pi_n)^*$  such that for any data word $(w, \sim)$ over $\Gamma$:
\begin{align*}
	w \otimes X \in L \quad \mbox{iff} \quad (w \otimes v) | X  \in K, \quad \mbox{ for any class }X.
\end{align*}
\end{lemma}
\begin{proof}(sketch)
	Let $\Aa$ be a deterministic automaton recognizing $L$. 
	Since $L$ is local,  for any two $a,b \in \Gamma$, the transitions of $\Aa$ over $(a,0)$ and $(b,0)$ 
	may be assumed to be the same. 
	Intuitively, only the number of consecutive positions outside of $X$ matters. Furthermore, as $\Aa$ is finite, this number can only be measured up to some finite threshold, and then modulo some number. This information is stored in the profile.
\end{proof}

	
	\begin{lemma}
	\label{c:profilecheck}
		For any $n \in \Nat$ there is a data automaton, with input alphabet $\Sigma \times \Pi_n$, which accepts a data word 
		$(w \otimes v, \sim)$ if and only if $v$ is the $n$-profile of $(w, \sim)$.
	\end{lemma}


\subsection{$\mathscr A_2$ versus $\mathscr C_2$.}
The relationship between Presburger automata and commutatively local class automata,
analogous to Propositions~\ref{prop:A0vsC0} and~\ref{prop:data-petri}, follows from results of~\cite{BojanczykJACM09}
specialized to data words.



\subsection{$\mathscr A_3$ versus $\mathscr C_3$}
	We now move to the last of the three decidable restrictions: gainy counter automata, and class automata with tail class conditions. Case $i=3$ of Theorem~\ref{thm:classification} will be a consequence of Propositions~\ref{prop:data-gainy} and~\ref{prop:tail-alternating} below. These propositions talk about alternating one register automata, which we define and discuss in more detail shortly. 
	
	\begin{proposition}[\cite{DBLP:journals/tocl/DemriL09}]
        \label{prop:data-gainy}The following language classes are equal.
		\begin{enumerate}
			\item Languages of words without data recognized by gainy counter automata.
			\item Projections of languages of data words recognized by alternating one register automata.
		\end{enumerate}
	\end{proposition}
	
Suppose $\pi : \Sigma \to \Gamma$.
% is a function from an input alphabet to an output alphabet, which we call a relabeling. 
If $K$ is a set of data trees over $\Sigma$, we write $\pi(K)$ for the set of data trees 
over $\Gamma$ obtained from $K$ by keeping the data and  replacing the labels using $\pi$. 
Any such $\pi(K)$ we call a relabeling of $K$. Note that unlike with projections, we do not erase any positions.

	\begin{proposition}\label{prop:tail-alternating}
		The following languages classes are equal:
		% conditions are equivalent to a language $L$ of data words.
		\begin{iteMize}{$\bullet$}
			\item Languages of data trees recognized by class automata with a tail class condition.
			\item Relabelings of languages of data trees recognized by alternating one register automata.
	\end{iteMize}		\end{proposition}
	
The two propositions give case $i=3$ of Theorem~\ref{thm:classification}, since the composition of a relabeling and a projection is a projection.
	
% \end{proof}

Note that the two propositions imply decidability of the emptiness problem for languages recognized by class automata with tail class condition.
To decide emptiness of such language $L$ do the following  steps. First, apply Proposition~\ref{prop:tail-alternating} to compute a relabeling $\pi$ and a language $K$ recognized by an alternating one register automaton, such that $L=\pi(K)$. Next, apply Proposition~\ref{prop:data-gainy} (more precisely, its tree variant from~\cite{DBLP:conf/lics/JurdzinskiL07}) to compute a gainy counter automaton (for trees) whose emptiness is equivalent to emptiness of $K$. Finally, use results on gainy counter automata for trees from~\cite{DBLP:conf/lics/JurdzinskiL07} to decide emptiness of the gainy counter automaton for trees.

\input{tail}


\removed{
\begin{proposition}
	\label{prop:local-equivalents} Class local, strongly class local, and very strongly class 
        local class automata are all equivalent to data automata. 
\end{proposition}
\removed{ 
\begin{iteMize}{$\bullet$}
	\item what is the first position in $\set{i+1,\ldots,i+n}$ with the same data value as $i$. 
          The possibles values are $+1,\ldots,+n$ and $\bot$. 
	\item 
\end{iteMize}
}

For a word $w \in \Sigma^*$ and two positions $x \le y$ in the word, we define $runs(w,x,y)$ to be 
the set of state pairs $(p,q)$ such that $\Aa$ has a run over the infix of $w \otimes $

We define $\delta_\mu$ to a word over alphabet $Q \times Q \cup Q $, which on position $x$ has the following information: 
\begin{iteMize}{$\bullet$}
	\item If $y$ is the first position after $x$ in the same class, then the label of $\delta_\mu$ in $x$ is 
	\begin{align*}
		runs(w,x+1,y-1) \subseteq Q \times Q. 
	\end{align*}
	\item If $x$ is the last position in its class, then the label of $\delta_\mu$ in $x$ is 
	\begin{align*}
		\set{p : (p,q) \in runs(w,x+1,|w|)} \subseteq Q. 
	\end{align*}
\end{iteMize}

Let $n,k \in \Nat$. Consider a number $x \in \Nat$ and a set $X \subseteq \Nat$ The $n$-profile 
of a position $x$ in a word $w \otimes X$ consists of two numbers: Let $L$ be a class local language.

} 


\removed{
%\removed
\sredniparagraph{Summary} The diagram below summarized all restricted classes of class automata mentioned in this section, together with their relationship with data automata and register automata. The arrows represent strict inclusions. We restrict to data words only, as the case of words is better understood.
\[ \xymatrix@=10pt{ & \txt{\bf class} & \\
\txt{\bf class local class\\(data automata)} \ar[ru] & & \txt{\bf tail class} \ar[lu] \\
\txt{\bf commut.\\
\bf class local class} \ar[u] & \txt{nondeterministic\\(multiple) register} \ar[lu]_{\cite{BjorklundS07}} & \txt{alternating\\
one register} \ar[u]_{\text{Thm.~\ref{thm:ara-to-tail}}} } \]
Table~\ref{table:subclasses}  
gives an overview of expressive power of all subclasses considered. The first issue we focus on is what logics over data words are captured by the automata. The second column in Table~\ref{table:subclasses} summarizes the results of this paper and of~\cite{BojanczykLICS06}, \cite{DBLP:journals/tocl/DemriL09} and~\cite{}.

The second issue is how expressible is the class of languages of words (without data) obtained by erasing the data labeling. Intriguingly, in each case the class is characterized as the languages recognized by an important model of computation, namely vector addition systems (Petri nets)~\cite{BojanczykLICS06}, incrementing errors ('gainy') counter machines~\cite{DBLP:journals/tocl/DemriL09}, or Presburger automata~\cite{}.
}


==> lazic.tex <==


\newcommand{\nodeval}[1]{#1_{\sim}}
\newcommand{\dom}{\mathrm{dom}}


\section{Decidability of tail class automata}

\label{sec:emptiness-of-ara}
We now prove that emptiness is decidable for tail class automata.
\begin{theorem}
	\label{thm:tail-decidable} Emptiness is decidable for tail class automata. 
\end{theorem}
Note that this theorem follows from the previous results.
To decide emptiness of the language $L$ of a tail class automaton, do the following  steps. First, apply Proposition~\ref{prop:tail-alternating} to compute a relabeling $\pi$ and a language $K$ recognized by an alternating one register automaton, such that $L=\pi(K)$. Next, apply Proposition~\ref{prop:data-gainy} (more precisely, its tree variant from~\cite{DBLP:conf/lics/JurdzinskiL07}) to compute a gainy counter automaton (for trees) whose emptiness is equivalent to emptiness of $K$. Finally, use results on gainy counter automata for trees from~\cite{DBLP:conf/lics/JurdzinskiL07} to decide emptiness of the gainy counter automaton for trees.

We give the proof below aiming at a self-contained presentation,
as we do not to use any external results to show that  emptiness is decidable for alternating one register automata, or for tail class automata. We would like to underline, however, that none of the ideas here are substantially different from the ones in the original papers on alternating one register automata. 

%Instead of giving a new proof, out intention is rather to relate different models in a common framework.
% In this section we show that emptiness is decidable for tail class automata.

Fot the rest of this section fix a tail class automaton $\Tt$. 
Let $f$ be the transducer, and let $\Aa$ be a tree automaton
%, call it the \emph{tail automaton},  
recognizing the tail condition. Let $P$ and $Q$ be the state spaces of $f$ and $\Aa$, respectively.

\subsection{Profiles}
A \emph{profile} is a pair consisting of a \emph{transducer state $p \in P$} and an \emph{obligation set $S$}, which is a finite subset of $Q \times D$. The rough idea is that a profile represents  run of $\Tt$ in the moment that it enters a node $x$  from its parent. The transducer  state represents the state of the transducer in $x$, while each pair $(q,d)$ in the obligation set represents a  run of the automaton $\Aa$ that was started for a class tail of an ancestor of $x$ with data value $d$. A more precise definition is presented below.

In the following we write $\Aa(q)$ for the automaton$\Aa$ with initial state changed to  $q$,  likewise  $f(p)$ for the transducer.
A profile $(p,S)$ is called \emph{satisfiable} if there exists a data tree $t \otimes \mu$ and
\begin{enumerate}
	\item A tree $s$ output by  $f(p)$.
	\item For each node $x$ in $s$, a run $\rho_x$ of $\Aa$ on the class tail of $x$ in $s \otimes \mu$.
	\item For each  $(q,d) \in S$, a  run $\rho_{(q,d)}$ of $\Aa(q)$ on  $s \otimes \mu^{-1}(d)$.
\end{enumerate}
Emptiness of $\Tt$ is equivalent to satisfiability of the \emph{initial profile}, where the transducer state is the initial state of the transducer, and the obligation set is empty. 
The rest of Section~\ref{sec:emptiness-of-ara} is devoted to an algorithm that decides if a given profile is satisfiable.



\subsection{Well structured transition systems}

\newcommand{\compl}[1]{\neg #1}

Consider an enumerable set, which we will call a \emph{domain}.
A \emph{transition system} on the domain  is a function $f$ that maps each element  $x$ of the domain to a nonempty family of subsets of the domain. A \emph{derivation}  is a finite tree whose nodes are labeled by elements of the domain, such that for each node with label $x$, the labels in the children of $x$ form a set from $f(x)$.  We write $f^*$ for the set of elements in the domain that have  (i.e.~appear in the root of) a derivation. 

%The derivation depth $|x|$ of an element $x \in f^*$ is the smallest depth of its derivations. For 
%instance, $|x|=1$ if and only if $\emptyset \in f(x)$. 

A transition system $f$ is called \emph{computable} if $f$ maps each element
to a \emph{finite} family of \emph{finite} subsets of the domain, and $f$ is a computable function.

A binary relation $R$ over the domain is called a \emph{downward simulation}  
if for any $(y, x) \in R$ and any  $X \in f(x)$, there is some $Y \in f(y)$ such that 
each element of $Y$ is related by $R$ to some element of $X$:
for each $y' \in Y$ there is $x' \in X$ with $(y', x') \in R$. 

\begin{lemma}
\label{lem:simulation}
If a downward simulation R contains a pair $(y, x)$ and $x \in f^*$ then $y \in f^*$ and  $|y| \le |x|$.
\end{lemma}

A transition system is \emph{monotone} if its domain is equipped with 
a partial order $\le$ that is a downward simulation.
By Lemma~\ref{lem:simulation} in a monotone transition system the set
$f^*$ is downward-closed, and thus its complement $\compl{f^*}$ is upward closed.

\begin{theorem}\label{thm:wqo}
	Consider an enumerable domain with  a computable, well founded order without infinite antichains. 
For any computable and monotone transition system $f$,  membership in $f^*$ is decidable.
\end{theorem}
\begin{proof}
	For an element $x$ of the domain  we run two algorithms in parallel. 
	The first algorithm enumerates all  derivations and terminates if it finds one with $x$ in the root.
Thus the algorithm  terminates if and only if $x$ belongs to $f^*$.
	

	\newcommand{\upward}[1]{#1^\uparrow}
	
	The second algorithm enumerates all finite antichains in the domain and terminates if it finds an antichain $Z$  that such that $x$ belongs to the upward closure of $Z$, call it $\upward Z$, and $Z$ satisfies the following property (*): 
for any element $z \in Z$, every set in $f(z)$ has nonempty intersection with $\upward Z$. 
We now show that this algorithm terminates if and only if $x$ does not belong to $f^*$.  

%	\begin{iteMize}
%		\item 
Suppose  that $x$ does not belong to $f^*$. 
We claim that the algorithm succeeds; one possible set $Z$ produced by the algorithm is all
minimal elements in the complement of $f^*$. Since the order has no infinite antichains, 
$Z$ is finite.   By well foundedness, the complement of $f^*$ equals $\upward Z$.
Thus $Z$ satisfies property (*) and $x \in \upward Z$. 

%				\item 
Suppose  that $x$ belongs to $f^*$. We claim that the upward closure $\upward Z$ of any  antichain $Z$  satisfying (*) contains no elements of $f^*$, and hence the algorithm must fail. 
For the proof we will use a bit of duality of induction and coinduction.

The set $f^*$ is the smallest set $\cal X$ with the property that
whenever $f(x)$ contains a set X with $X \subseteq {\cal X}$ then
$x \in {\cal X}$.
Thus $f^*$ is the smallest (pre-)fixed point of the mapping:
\[
{\cal F} : {\cal X} \mapsto \{ x : \text{ some set in } f(x) \text{ is included in } {\cal X} \},
\]
ie., the smallest ${\cal X}$ with ${\cal F}({\cal X}) \subseteq {\cal X}$.
By duality, the complement of $f^*$ is the greatest (post-)fixed point of the mapping
${\cal X} \mapsto \compl{{\cal F}(\compl{\cal X})}$; i.e.,
the greatest ${\cal X}$ with ${\cal X} \subseteq \compl{{\cal F}({\compl{\cal X}})}$;
i.e., the greatest ${\cal X}$ such that
whenever $x \in {\cal X}$ then
each set in $f(x)$ has nonempty intersection with ${\cal X}$.

Now we are ready to argue that if $Z$ satisfies (*) then $\upward Z$ is 
included in $\compl{f^*}$. Indeed, by monotonicity it follows
that $\upward Z$ satisfies (*): for every $z \in \upward Z$,
every set in $f(z)$ has nonempty intersection with $\upward Z$.
Thus $\upward Z$ is a post-fixed point,
$\upward Z \subseteq \compl{{\cal F}(\compl{\upward Z})}$, and hence necessarily 
is included in the greatest one.
\end{proof}


\subsection{Profiles form a transition system}
\label{sec:profiles-ts}

\newcommand{\quot}{\widehat}
\newcommand{\lleft}{0}
\newcommand{\rright}{1}
\newcommand{\svector}[1]{\langle #1 \rangle}
\newcommand{\qinit}{q_\text{init}}

In this and in the next section we apply the machinery of Theorem~\ref{thm:wqo}  to decide which profiles are satisfiable, completing the decision procedure for emptiness of  tail class automata. 
Our aim is first to define an ordered domain and a transition system $f$,  and then its quotient $\quot f$
that satisfies the assumptions of Theorem~\ref{thm:wqo}, and such  that satisfiable profiles 
can be computed on the basis of testing membership in ${\quot f}^*$.

The domain of $f$ will contain all profiles; $f$ itself we define below.
The definition of $f$ is designed so that a data tree that makes a profile satisfiable 
is essentially a derivation of this profile, and vice versa
(cf.~Lemma~\ref{lem:satisfiable-reachable} below). 

A profile $(p, S)$ we call \emph{accepting} if 
$p$ as well as all states appearing in $S$ are accepting.
If a profile $x = (p, S)$ is accepting then let $f(x)$ contain only $\emptyset$.
Otherwise, $f(x)$ will contain all the sets $\{ (p_\lleft, S_\lleft), (p_\rright, S_\rright) \}$, 
of size at most two each, that arise as an outcome of the following nondeterministic 'procedure':
\begin{iteMize}{$\bullet$}
\item
Choose an input letter $a$ of $f$, 
a transition $p, a \to b, p_\lleft, p_\rright$ thereof, and a data value $\bar d$.
\item
For each $(q, d) \in S \cup \{ (\qinit, \bar d) \}$, where $\qinit$ is the initial state of $\Aa$,
choose a transition of $\Aa$
	\begin{eqnarray*}
		\begin{array}{rclll}
			q, (b,1) & \to & q_\lleft,q_\rright & \qquad & \mbox{if $d=\bar d$}\\
			q, (b,0) & \to & q_\lleft,q_\rright & & \mbox{if $d \neq \bar d$}
		\end{array}
	\end{eqnarray*}
and add $(q_\lleft, d)$ to $S_\lleft$ and $(q_\rright, d)$ to $S_\rright$.
\end{iteMize}


\begin{lemma}
\label{lem:satisfiable-reachable}
Satisfiable profiles are exactly $f^*$.
\end{lemma}

The profiles are ordered coordinatewise, 
with the first coordinate (states of the transducer) ordered discretely (all states are incomparable),
and the second coordinate (obligations) ordered by inclusion.
%
\begin{lemma}
\label{lem:monotone-concr}
The transition system $f$ is monotonne.
\end{lemma}


\subsection{Abstractions of profiles form a well-structured transition system}
\label{sec:wsts}

Now we define the well structured transition system $\quot f$.
Elements of the domain will not be profiles, but  isomorphism classes of profiles, 
in the following sense. 
Two  profiles are called \emph{isomorphic} if they have the same transducer state 
and there is a bijection on data values that maps one obligation set to the other. 
It is not difficult to see that the isomorphism class of $(p,S)$ is identified by its 
\emph{abstraction} $(p,[S])$, where the vector
\begin{align*}
	[S] \in  \Nat^{P(Q) \setminus \set \emptyset }\ ,
\end{align*}
called the \emph{abstraction of $S$},  stores on coordinate $Q' \subseteq Q$ 
the number of data values in the set
\begin{align*}
\set{d \in D : Q' = \set{q : (q,d) \in S}}.
\end{align*}

The domain of $\quot f$ will consist of abstractions of profiles;
in particular, the domain is enumerable.
%
Since isomorphic profiles are equivalently satisfiable, this abstraction is not a problem: 
it makes sense to talk about satisfiable abstractions. 

The transition function $\quot f$ is defined by projecting the transition  function $f$:
if $w = [S]$ is an abstraction of the obligation set $S$, then
${\quot f}(p, w)$ contains precisely those sets that are obtained
by abstraction of some set $X$ from $f(p, S)$; by abstraction of $X$ 
we mean here the set of profile abstractions obtained by 
replacing each profile $(p', S')$ appearing in $X$ with 
its abstraction $(p', [S'])$.

The following lemma together with Lemma~\ref{lem:satisfiable-reachable}
reduces emptiness of tail class automata to testing ${\quot f}^*$.
\begin{lemma}
A profile is in $f^*$ if and only if its abstraction is in ${\quot f}^*$.
\end{lemma}
\begin{proof}
For both directions we may use Lemma~\ref{lem:simulation} 
applied to the disjoint union of $f$ and $\quot f$; as the downward simulation
we will use either the relation $R$ containing all pairs
(a profile, its abstraction),
% = \{ (x, [x]) : x \text{ is a profile} \}$,
or the inverse relation $R^{-1}$, respectively.
It remains to show that both $R$ and $R^{-1}$ are downward simulations.

Observe that the isomorphism of profiles satisfies a stronger property,
which we call a \emph{2-level bisimulation}:
whenever $x$ and $y$ are isomorphic and $X \in f(x)$, there is 
$Y \in f(y)$ such that $X$ and $Y$ witness the following 
\emph{1-level bisimulation} condition:
for any $x' \in X$ there is $y'\in Y$ isomorphic to $x'$; and vice versa,
for any $y' \in Y$ there is $x' \in X$ isomorphic to $y'$.
%
% The profile isomorphism has been defined as the union of such relations, for all bijections $i$,
% and is thus a bisimulation as well.
%

In consequence, the relation $R$ is a 2-level bisimulation too.
Thus both $R$ and $R^{-1}$ are downward simulations indeed.
\end{proof}

The transition function $\quot f$ maps always an abstraction $x$
to a finite family of finite sets of abstractions,
and ${\quot f}(x)$ is computable, for a given $x$,
by simulating the nondeterministic procedure given in Section~\ref{sec:profiles-ts}.
Thus we have:

\begin{lemma}\label{lem:computable-abstr}
The transition system $\quot f$ is computable.
\end{lemma}

The order on abstractions of obligation sets is 
defined by projecting the inclusion order on obligation sets:
$w \leq w'$ if $w = [S]$, $w' = [S']$ for some obligation sets $S \subseteq S'$.
Accordingly we define the order on abstractions of profiles:
$(p, w) \leq (p', w')$ if $p = p'$ and $w \leq w'$.
%
Directly by Lemma~\ref{lem:monotone-concr} and by the bisimulation property of
the profile isomorphism we get:
\begin{lemma}\label{lem:monotone-abstr}
The transition system $\quot f$ is monotone.
\end{lemma}

We complete the check-list of assumptions of Theorem~\ref{thm:wqo}
by showing the following:

\begin{lemma}\label{lem:order-computable}
The order $\leq$ is computable, well founded and has no infinite antichains.
\end{lemma}
\begin{proof}
Since there are finitely many transducer states, it suffices that these properties hold 
for the order on abstractions of obligation sets. 

Recall that abstractions of obligation sets are vectors of numbers 
indexed by nonempty subsets of $Q$. 
Note that the order on abstractions of obligation sets we use here, is not the same as 
the classical coordinatewise order on vectors of numbers, call it $\preceq$. 
	
To show computability, we give the following alternative definition of $\le$. For two  abstractions $v,w$ of obligation sets, we have $v \le w$  if and only if $v$ can be reached from $w$ by a finite number of steps of the form: choose a coordinate $R \subseteq Q$ and an element $q \in R$, decrement the vector on coordinate $R$; and then increment the vector  on coordinate $R \setminus \set q$ if
$R \setminus \set q$ is nonempty.

This alternate definition also shows that the order is well founded: it is impossible to do an infinite sequence of such steps.
% since each step decreases the sum of coordinates.

Finally, we want to show that $\le$ has no infinite antichains. It is not hard to see that $v \preceq w$ implies $v \le w$. It is well known that  $\preceq$ has no infinite antichains, and hence the same must hold for $\le$.
\end{proof}













